Low-count Time Series Anomaly Detection

Low-count time series describe sparse or intermittent events, which are prevalent in large-scale online platforms that capture and monitor diverse data types. Several distinct challenges surface when modelling low-count time series, particularly low signal-to-noise ratios (when anomaly signatures are provably undetectable), and non-uniform performance (when average metrics are not representative of local behaviour). The time series anomaly detection community currently lacks explicit tooling and processes to model and reliably detect anomalies in these settings. We address this gap by introducing a novel generative procedure for creating benchmark datasets comprising of low-count time series with anomalous segments. Via a mixture of theoretical and empirical analysis, our work explains how widely-used algorithms struggle with the distribution overlap between normal and anomalous segments. In order to mitigate this shortcoming, we then leverage our findings to demonstrate how anomaly score smoothing consistently improves performance. The practical utility of our analysis and recommendation is validated on a real-world dataset containing sales data for retail stores.

==> problem_statement.tex <==
\section{Problem Statement}

% In the general TSAD setting, we observe a series of values, $x_{1:t} = \left[ x_1, \dots, x_t\right]$, which describe a system of interest at time steps $\{1,\dots, t\}$.
% The objective is to generate an anomaly score $a_t(x_{1:t})$ at each time step based on how observed values deviate from expected patterns.
% A threshold scheme can then be applied to the anomaly scores to convert them into a sequence of binary labels $\left[s_1, \dots, s_t\right]$ indicating whether a deviation is alarm-worthy or not.

